Rethinking Stateful Tool Use in Multi-Turn Dialogues: Benchmarks and Challenges

Existing benchmarks that assess Language Models (LMs) as Language Agents (LAs) for tool use primarily focus on stateless, single-turn interactions or partial evaluations, such as tool selection in a single turn, overlooking the inherent stateful nature of interactions in multi-turn applications. To fulfill this gap, we propose \texttt{DialogTool}, a multi-turn dialogue dataset with stateful tool interactions considering the whole life cycle of tool use, across six key tasks in three stages: 1) \textit{tool creation}; 2) \textit{tool utilization}: tool awareness, tool selection, tool execution; and 3) \textit{role-consistent response}: response generation and role play. Furthermore, we build \texttt{VirtualMobile} -- an embodied virtual mobile evaluation environment to simulate API calls and assess the robustness of the created APIs\footnote{We will use tools and APIs alternatively, there are no significant differences between them in this paper.}. Taking advantage of these artifacts, we conduct comprehensive evaluation on 13 distinct open- and closed-source LLMs and provide detailed analysis at each stage, revealing that the existing state-of-the-art LLMs still cannot perform well to use tools over long horizons.

==> tables/api_list.tex <==
\begin{table}[!t]
%\setlength{\abovecaptionskip}{5pt}   
\setlength{\belowcaptionskip}{0pt}
    \centering
    \begin{adjustbox}{max width=0.5 \textwidth}
    \begin{tabular}{l|c}
    \toprule
    Restaurant & Weather
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{The list of APIs}
    \label{tab:api_list}
\end{table}

==> tables/app_list.tex <==
\begin{table}[!t]
%\setlength{\abovecaptionskip}{5pt}   
\setlength{\belowcaptionskip}{0pt}
    \centering
    \begin{adjustbox}{max width=0.5 \textwidth}
    \begin{tabular}{l|c}
    \toprule
    Restaurant & Weather
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{The list of APPs}
    \label{tab:app_list}
\end{table}

==> tables/before.tex <==
\begin{table*}[!t]
%\setlength{\abovecaptionskip}{5pt}  
    \setlength{\belowcaptionskip}{0pt}
    \centering
    \begin{adjustbox}{max width=0.8 \textwidth}
    \begin{tabular}{l| c| ccc | ccc}
    \toprule
    \multirow{2}{*}{\textbf{Models}} & \multirow{2}{*}{\textbf{Creation}} & \multicolumn{3}{c|}{\textbf{Actions}} & \multicolumn{3}{|c}{\textbf{Responses}} \\    
    % dynamic / multi-turn?
    \cline{3-8} & & \textbf{Acc} ($\uparrow$) & \textbf{Tools} ($\downarrow$) & \textbf{No tools} ($\downarrow$) & BLEU ($\uparrow$) & R.L ($\uparrow$) & Role ($\uparrow$) \\
    \hline
    ChatGLM3-6B & 31.5 & 58.9 & 8.2 & 32.9 & 7.8 & 7.5 & 4.8 \\
    LLaMA2-7B & 33.2 & 63.5 & 4.3 & 32.2 & 6.8 & 5.7 & 6.2 \\
    QWen1.5-7B & 21.9 & \underline{68.9} & \textbf{2.5} & 28.6 & 8.0 & 7.4 & 7.0 \\
    Mistral-7B & 11.4 & 42.5 & 29.7 & 27.8 & 8.0 & 7.1 & 6.7 \\
    LLaMA3-8B & 62.2 & 46.3 & 20.8 & 32.9 & 8.3 & 7.7 & 7.0 \\
    
    \hdashline
    
    LLaMA2-13B & 48.8 &  47.1 & 19.6 & 33.3 & 7.7 & 6.4 & 6.5 \\
    Vicuna-13B & - & 64.5 & 10.5 & 25.0 & 10.1 & 11.5 & 6.0 \\
    QWen1.5-14B & 27.9 & 51.7 & 21.8 & 26.5 & 9.3 & 10.9 & 7.5 \\

    \hdashline
    QWen1.5-72B & 49.7 & \textbf{75.5} & 7.3 & \underline{17.2} & \underline{10.8} & \textbf{15.3} & 7.4 \\
    LLaMA2-70B & 23.0 & 34.7 & 34.2 & 31.2 & 8.5 & 10.7 & 6.2 \\
    LLaMA3-70B & \textbf{69.7} & 40.2 & 39.2 & 20.6 & 9.0 & 11.3 & \underline{7.7} \\
    
    \hdashline
    
    GPT-3.5 & 63.3 & 67.9 & \underline{4.8} & 27.3 & 10.2 & 11.9 & 6.7 \\
    GPT-4o & \underline{66.7} & 63.5 & 19.9 & \textbf{16.7} & \textbf{11.4} & \underline{14.5} & \textbf{8.3} \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \vspace{2mm}
    \caption{The results \textbf{before} and \textbf{after} the tool utilization of different LLMs. \textbf{Tools}: The rates of cases that LLMs should use tool but the action does not invoke it (false negative); \textbf{No Tools}: The rates of cases that LLMs should not use tool but the action invoke tool call or invoke other types of \textit{non-tool} actions (false positive).}
    \label{tab:before_exp}
\end{table*}

==> tables/during.tex <==
\begin{table*}[!t]
%\setlength{\abovecaptionskip}{5pt}   
\setlength{\belowcaptionskip}{0pt}
    \centering
    \begin{adjustbox}{max width=0.8 \textwidth}
    \begin{tabular}{l| ccc | cccc}
    \toprule
    \multirow{2}{*}{\textbf{Models}} & \multicolumn{3}{c}{\textbf{Tool Selection}} & \multicolumn{4}{|c}{\textbf{Tool Execution}} \\    
    % dynamic / multi-turn?
    \cline{2-8} & \textbf{Acc} ($\uparrow$) & \textbf{Recall} ($\uparrow$) & \textbf{Error} ($\downarrow$) & \textbf{Acc} ($\uparrow$) & \textbf{Miss} ($\downarrow$) & \textbf{Match} ($\downarrow$) & \textbf{API} ($\downarrow$) \\
    \hline
    ChatGLM3-6B & 32.8 & 40.4 & (6.4/27.7) & 6.8 & 24.9 & 14.5 & 53.8 \\
    
    LLaMA2-7B & 27.4 & 38.2 & (17.1/33.3) & 7.0 & 29.7 & 18.4 & 44.8 \\
    
    QWen1.5-7B & 54.7 & 76.8 & (0.8/28.9) & 11.3 & 40.2 & 26.4 & 22.1 \\
    
    Mistral-7B & 51.8 & 57.6 & (0.4/5.5) & 22.6 & 22.8 & 13.1 & 41.4 \\
    
    LLaMA3-8B & 61.4 & 64.6 & (1.2/4.0) & 45.6 & 9.3 & 12.0 & 33.0 \\
    
    \hdashline
    
    LLaMA2-13B & 51.1 & 59.9 & (4.1/13.1) & 11.7 & 38.5 & 17.2 & 32.5  \\
    
    Vicuna-13B & 62.9 & 67.1 & (2.7/9.4) & 12.3 & 38.6 & 20.2 & 28.9 \\
    
    QWen1.5-14B & 55.6 & 46.8 & (11.3/3.7) &  21.8 & 23.7 & 25.2 & 29.3 \\

    \hdashline
    QWen1.5-72B & \underline{71.9} & \underline{84.2} &  (0.2/11.5) & 49.3 & 18.1 & 17.2 & 15.4 \\
    
    LLaMA2-70B & 57.8 & 70.6 & (0.6/1.0) &  32.6 & 30.0 & \underline{10.2} & 27.2 \\
    
    LLaMA3-70B & 57.1 & 82.6 & (\underline{\textbf{0.0}/\underline{0.4}}) & 68.1 & \textbf{6.6} & \textbf{7.9} & 17.4  \\
    
    \hdashline
    
    GPT-3.5 & 50.0 & 68.6 &  (\underline{0.1}/27.1) & 42.6 & 9.6 & 16.5 & 31.3  \\
    GPT-4o & \textbf{77.8} & \textbf{91.4} & (0.9/\textbf{0.3}) & \textbf{68.7} & \underline{9.3} & 14.2 & \textbf{7.8} \\
    % GPT-4o & 69.0 & 84.0 & (0.7/3.7) & 55.2 & 13.8 & 16.8 & 14.2 \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{The results \textbf{during} the tool utilization of different LLMs. We list (API parse error / unnecessary tool calls) at the Error column for tool selection. }
    \label{tab:during_exp}
\end{table*}

==> tables/human_eval.tex <==
\begin{table}[!t]
%\setlength{\abovecaptionskip}{5pt}  
    \setlength{\belowcaptionskip}{0pt}
    \centering
    \begin{adjustbox}{max width=0.5 \textwidth}
    \begin{tabular}{l|c}
    \toprule
    \textbf{Models} \hspace{16mm} & \hspace{8mm} \textbf{Score} \hspace{8mm} \\
    \hline
    ChatGLM3-6B & 1.64 \\
    LLaMA2-7B & 1.25 \\
    QWen1.5-7B & 2.82 \\
    Mistral-7B & 2.28 \\
    LLaMA3-8B & 2.69 \\
    
    \hdashline
    
    LLaMA2-13B & 2.17 \\
    Vicuna-13B & 2.59 \\
    QWen1.5-14B & 2.44 \\

    \hdashline
    QWen1.5-72B & 3.37 \\
    LLaMA2-70B & 2.56  \\
    LLaMA3-70B & 2.98 \\
    
    \hdashline
    
    GPT-3.5 & \underline{3.42} \\
    GPT-4o & \textbf{3.56} \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{The results of human evaluation on the response generation task. The inter-agreement is around 80\%.}
    \label{tab:human_eva}
    
\end{table}

==> tables/memory_exp.tex <==
\begin{table*}[!t]
%\setlength{\abovecaptionskip}{5pt}   
\setlength{\belowcaptionskip}{0pt}
    \centering
    \begin{adjustbox}{max width=1.0 \textwidth}
    \begin{tabular}{l | ccc}
    \toprule
    % dynamic / multi-turn?
    \textbf{Model} & \textbf{Acc} ($\uparrow$) & \textbf{Memory} ($\downarrow$) & \textbf{No Memory} ($\downarrow$)  \\
    \hline
    ChatGLM3-6B & 56.9 & 21.2 & 21.9 \\
    LLaMA2-7B & 27.8 & 0.4 & 71.9 \\
    QWen1.5-7B & 46.8 & 20.4 & 32.8 \\
    Mistral-7B & 59.4 & 23.2 & 17.4 \\
    LLaMa3-8B & 21.7 & 11.8 & 66.5 \\
    \hdashline
    LLaMA2-13B & 43.1 & 16.8 & 40.1 \\
    Vicuna-13B & 56.8 & 18.5 & 24.7 \\
    QWen1.5-14B & 19.1 & 9.1 & 71.8 \\
    \hdashline
    QWen1.5-72B & 22.3 & 12.5 & 65.1 \\
    LLaMA2-70B & 19.5 & 9.9 & 70.7 \\
    LLaMA3-70B & 19.1 & 11.8 & 69.1 \\
    \hdashline
    GPT-3.5 & 54.4 & 21.6 & 24.0 \\
    GPT-4o & 22.4 & 13.3 & 64.3 \\
    \bottomrule
    \end{tabular}
    \end{adjustbox}
    \caption{The Performance of different LLMs to utilize \texttt{Memory} App to retrieve user memory/persona to generate personalized responses in open-domain setting. The \textbf{Memory} column stands for cases which require to use user memory but the agent decide not to use, and \textbf{No Memory} means the opposite cases.}
    \label{tab:memory_exp}
\end{table*}
